The clustering of $z > 7$ galaxies: Predictions from the BLUETIDES simulation

We study the clustering of the highest-z galaxies (from ~ $0.1$ to a few tens Mpc scales) using the BLUETIDES simulation and compare it to current observational constraints from Hubble legacy and Hyper Suprime Cam (HSC) fields (at $z=6-7.2$). With a box length of $400$ $Mpc/h$ on each side and $0.7$ trillion particles, BLUETIDES is the largest high resolution cosmological hydrodynamic simulation to date ideally suited for studies of high-z galaxies. We find that galaxies with magnitude $m_{UV}<27.7$ have a bias ($b_g$) of $8.1\pm 1.2$ at $z=8$, and typical halo masses $M_H \gtrsim 6\times10^{10} M_{\odot}$. Given the redshift evolution between $z=8$ to $z=10$ ($b_g\propto(1+z)^{1.6}$), our inferred values of the bias and halo masses are consistent with measured angular clustering at $z \sim 6.8$ from these brighter samples. The bias of fainter galaxies (in the Hubble legacy field at $H_{160} \lesssim29.5$) is $5.9\pm0.9$ at $z=8$ corresponding to halo masses $M_H \gtrsim 10^{10} M_{\odot}$. We investigate directly the 1-halo term inthe clustering and show that it dominates on scales $r \lesssim 0.1$ Mpc/$h$ ($\Theta \lesssim 3"$) with non-linear effect at transition scales between the 1-halo and 2-halo term affecting scales 0.1 $\lesssim r \lesssim $ 20 Mpc/$h$ ($3"\lesssim \Theta \lesssim 90"$). Current clustering measurements probe down to the scales in the transition between 1-halo to 2-halo regime where non-linear effects are important. The amplitude of the 1-halo term implies that occupation numbers for satellites in \texttt{BLUETIDES} are somewhat higher than standard HODs adopted in these analyses (which predict amplitudes in the 1-halo regime suppressed by a factor 2-3). That possibly implies a higher number of galaxies detected by JWST (at small scales and even fainter magnitudes) observing these fields.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
